Search for bottom squark pair production in proton--proton collisions at $\sqrt{s}=$13 TeV with the ATLAS detector

The result of a search for pair production of the supersymmetric partner of the Standard Model bottom quark ($\tilde{b}_1$) is reported. The search uses 3.2 fb$^{-1}$ of $pp$ collisions at $\sqrt{s}=$13 TeV collected by the ATLAS experiment at the Large Hadron Collider in 2015. Bottom squarks are searched for in events containing large missing transverse momentum and exactly two jets identified as originating from $b$-quarks. No excess above the expected Standard Model background yield is observed. Exclusion limits at 95% confidence level on the mass of the bottom squark are derived in phenomenological supersymmetric $R$-parity-conserving models in which the $\tilde{b}_1$ is the lightest squark and is assumed to decay exclusively via $\tilde{b}_1 \rightarrow b \tilde{\chi}_1^0$, where $\tilde{\chi}_1^0$ is the lightest neutralino. The limits significantly extend previous results; bottom squark masses up to 800 (840) GeV are excluded for the $\tilde{\chi}_1^0$ mass below 360 (100) GeV whilst differences in mass above 100 GeV between the $\tilde{b}_1$ and the $\tilde{\chi}_1^0$ are excluded up to a $\tilde{b}_1$ mass of 500 GeV.

==> VR_table.tex <==
\begin{table}[hb]
\begin{center}
\setlength{\tabcolsep}{0.0pc}
{\small
\caption{Fit results in the validation regions for an integrated luminosity of \intlumi.
The results are obtained from the control regions using the background-only fit (see text for details).
The individual uncertainties, including detector-related and theoretical systematic components, can be correlated and do 
not necessarily add up in quadrature to the total systematic uncertainty. }
\label{tab:fit_VR}
%%
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lrrr}
\noalign{\smallskip}\hline\noalign{\smallskip}
{\bf Validation region}         & VRmctA                    & VRmbbA                   & VRB     \\[-0.05cm]

\noalign{\smallskip}\hline\noalign{\smallskip}
%%

%%
Observed           & $41$              & $68$              & $76$                 \\
\noalign{\smallskip}\hline\noalign{\smallskip}
%%
Total background (fit)         & $54 \pm 7$          & $76 \pm 7$          & $72 \pm 7$             \\
\noalign{\smallskip}\hline\noalign{\smallskip}
%%
        \ttbar         & $36 \pm 7$          & $ 21 \pm 4$          & $47 \pm 6$            \\             
%%                                                                                                                                                  
        single top         & $4.6 \pm 2.1$          & $2.6 \pm 1.2$          & $3.9 \pm 0.6$     \\                
%%                                                                                                                                                  
        $W$+jets         & $2.9 \pm 0.8$          & $11 \pm 4$          & $6.4 \pm 3.4$            \\         
%%                                                                                                                                                  
        $Z$+jets         & $10.8 \pm 3.3$          & $35 \pm 6$          & $14.0 \pm 3.2$            \\
%%                                                                                                                                                  
        ``Other''         & $0.29 \pm 0.06$          & $5.4 \pm 0.6$          & $0.80 \pm 0.19$     \\
%%                                                                                                                                                  
 \noalign{\smallskip}\hline\noalign{\smallskip}                                                                 
%%                                                                                                                                                  
Total background (MC exp.)              & $53.7$          & $5.6$          & $68.1 $           \\
\noalign{\smallskip}\hline\noalign{\smallskip}                                                                  
%%                                                                                                                                                  
         \ttbar         & $37.3$          & $21.8$          & $47.5 $          \\
%%                                                                                                                                                  
         single top         & $5.6$          & $3.1$          & $3.9$       \\   
%%                                                                                                                                                  
         $W$+jets         & $2.4 $          & $9.4 $          & $6.4$           \\
%%                                                                                                                                                 
         $Z$+jets         & $8.0 $          & $26.3 $          & $9.4$            \\
%%                                                                                                                                                  
         ``Other''         & $0.29$          & $5.5$          & $0.8 $          \\
%%     \\


\end{tabular*}
%%%
}
\end{center}
\end{table}
%


==> auxiliary.tex <==
\section{Auxiliary material}
This is material that is to be made public and the material for the HepData database.

\subsection{Cutflows for SRA for a point with $m(\bone)=$700~\GeV\ and $m(\neut)=1$~\GeV}
\begin{small}
\begin{verbatim}
Total 			: 214.552
ETMiss Trigger 		: 203.758
Primary Vertex >= 1 	: 203.758
Jet/MET 		: 202.332
nLepton == 0  		: 200.668
nBaselineLepton == 0  	: 198.853
ETMiss > 250  		: 154.355
njets = 2 || 3 || 4 	: 123.219
pT(j1,j2) > (130, 50) 	: 121.238
pTj4 < 50 		: 99.459
JetMET dphi> 0.4 	: 88.667
nbjets == 2 		: 36.257
leading bs 		: 28.558
MET/mEff > 0.25 	: 27.824
m_bb > 200 		: 25.160
m_CT > 250 		: 20.815
m_CT > 350 		: 14.223
m_CT > 450 		: 8.185
\end{verbatim}
\end{small}

\subsection{Cutflows for SRB for a point with $m(\bone)=$400~\GeV\ and $m(\neut)=300$~\GeV}
\begin{small}
\begin{verbatim}
Total 			: 5873.184
ETMiss Trigger 		: 2970.814
Primary Vertex >= 1 	: 2970.814
Jet/MET 		: 2949.033
nLepton == 0  		: 2909.242
nBaselineLepton == 0  	: 2874.865
ETMiss > 400  		: 156.672
njets = 2 || 3 || 4 	: 105.633
pT(j1,j2) > (300, 50) 	: 89.310
pTj4 < 50 		: 69.835
Jet_MET dphi> 0.4 	: 51.436
Jet1_MET dphi> 2.5 	: 50.676
nbjets == 2 		: 13.063
secondary b 		: 10.521
MET/mEff > 0.25 	: 10.521
\end{verbatim}
\end{small}
\newpage

\subsection{Validation region yields}
~~
\input{VR_table}
\newpage


\subsection{Auxiliary plots for the data driven methods}
\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.49\textwidth]{figures/aux/mctjj_SRA_DD_ZfromGamma_v5.eps}
    \includegraphics[width=0.49\textwidth]{figures/aux/mctjj_SRA_DD_ZfromLight_v5.eps}
    \caption{Comparison between data and SM predictions for the \mct distribution in SRA. The data-driven predictions for the $Z$+jets background shown in these plots are evaluated using the alternative methods described in the text. Left: data-driven prediction derived from $\gamma$+jets. Right: data-driven prediction derived from $Z$+light jets processes.} 
    \label{fig:sbottom_aux_1}
  \end{center}
\end{figure}

\newpage

\subsection{Auxiliary material for the hepdata information}

\begin{figure}[htb]
  \begin{center}
%    \includegraphics[width=0.49\textwidth]{figures/aux/limit_combined_best.eps}
%    \includegraphics[width=0.49\textwidth]{figures/aux/sbottom_sigaccSRbest_text.eps}
    \includegraphics[width=0.65\textwidth]{figures/aux/limit_combined_bestSR.eps}
    \caption{Best expected signal region for each of the signal points studied.} 
    \label{fig:sbottom_aux_2}
  \end{center}
\end{figure}     

\begin{figure}[htb]
  \begin{center}

\includegraphics[width=0.45\textwidth]{figures/aux/limit_combined_UpperLimits.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/limitPlotSbottom_Sbottom_A250_UpperLimits.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/limitPlotSbottom_Sbottom_A350_UpperLimits.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/limitPlotSbottom_Sbottom_A450_UpperLimits.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/limitPlotSbottom_Sbottom_B_UpperLimits.eps}

    \caption{Cross-section upper limit for each of the signal points considered. From top to bottom, clockwise: best signal region and signal region SRA250, SR350, SR450, SRB, separately.}
    \label{fig:sbottom_aux_3}
  \end{center}
\end{figure}

\begin{figure}[htb]
  \begin{center}
\includegraphics[width=0.45\textwidth]{figures/aux/limit_combined_expCLs.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/limitPlotSbottom_Sbottom_A250_expCLs.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/limitPlotSbottom_Sbottom_A350_expCLs.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/limitPlotSbottom_Sbottom_A450_expCLs.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/limitPlotSbottom_Sbottom_B_expCLs.eps}
    \caption{Expected CLs for each of the signal points studied. From top to bottom, clockwise: best signal region and signal region SRA250, SR350, SR450, SRB, 
separately.}
    \label{fig:sbottom_aux_4}
  \end{center}
\end{figure}

\begin{figure}[htb]
  \begin{center}
\includegraphics[width=0.45\textwidth]{figures/aux/limit_combined_obsCLs.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/limitPlotSbottom_Sbottom_A250_obsCLs.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/limitPlotSbottom_Sbottom_A350_obsCLs.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/limitPlotSbottom_Sbottom_A450_obsCLs.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/limitPlotSbottom_Sbottom_B_obsCLs.eps}
\caption{Observed CLs for each of the signal points studied. From top to bottom, clockwise: best signal region and signal region SRA250, SR350, SR450, SRB, separately.}
    \label{fig:sbottom_aux_5}
  \end{center}
\end{figure}

%\begin{figure}[htb]
%  \begin{center}
%\includegraphics[width=0.45\textwidth]{figures/aux/truth_rate_bestSR.eps}
%\includegraphics[width=0.45\textwidth]{figures/aux/truth_rate_SRA250.eps}
%\includegraphics[width=0.45\textwidth]{figures/aux/truth_rate_SRA350.eps}
%\includegraphics[width=0.45\textwidth]{figures/aux/truth_rate_SRA450.eps}
%\includegraphics[width=0.45\textwidth]{figures/aux/truth_rate_SRB.eps}
%\caption{Event yields for each of the signal points studied. From top to bottom, clockwise: best signal region and signal region SRA250, SR350, SR450, SRB, separately.}
%    \label{fig:sbottom_aux_6}
%  \end{center}
%\end{figure}

\begin{figure}[htb]
  \begin{center}
\includegraphics[width=0.45\textwidth]{figures/aux/efficiency_recotruth_bestSR.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/efficiency_recotruth_SRA250.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/efficiency_recotruth_SRA350.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/efficiency_recotruth_SRA450.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/efficiency_recotruth_SRB.eps}
\caption{Reconstruction efficiency for each of the signal points studied. From top to bottom, clockwise: best signal region and signal region SRA250, SR350, SR450, SRB, separately.}
    \label{fig:sbottom_aux_7}
  \end{center}
\end{figure}

\begin{figure}[htb]
  \begin{center}
\includegraphics[width=0.45\textwidth]{figures/aux/truth_acceptance_bestSR.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/truth_acceptance_SRA250.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/truth_acceptance_SRA350.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/truth_acceptance_SRA450.eps}
\includegraphics[width=0.45\textwidth]{figures/aux/truth_acceptance_SRB.eps}
\caption{Acceptance for each of the signal points studied. From top to bottom, clockwise: best signal region and signal region SRA250, SR350, SR450, SRB, separately.}
    \label{fig:sbottom_aux_8}
  \end{center}
\end{figure}


\begin{figure}[htb]
  \begin{center}
   \includegraphics[width=0.65\textwidth]{figures/aux/syst_bestSR.eps}
    \caption{ Total experimental uncertainty for each of the signal points studied.} 
    \label{fig:sbottom_aux_9}
  \end{center}
\end{figure}



\begin{table}[ht!]
\begin{center}
\caption{Details of the signal samples generated.}
\label{tab:SampleDetails}
\begin{tiny}
\begin{tabular}{@{}cccc||cccc@{}}
 \toprule
   $m(\bone)$~[\gev] & $m(\neut)$~[\gev]  & MC evts (x1000) & x-sec~[pb] & $m(\bone)$~[\gev] & $m(\neut)$~[\gev]  & MC evts (x1000) & x-sec~[pb]   \\
            \midrule
250 & 230 & 488 & 21.595 & 250 & 245 & 496 & 21.595 \\
300 & 230 & 150 & 8.516 & 300 & 150 & 246 & 8.516 \\
300 & 280 & 98 & 8.516 & 300 & 295 & 99 & 8.516 \\
350 & 150 & 146 & 3.787 & 350 & 250 & 150 & 3.787 \\
350 & 330 & 597 & 3.787 & 350 & 345 & 589 & 3.787 \\
400 & 1 & 79 & 1.835 & 400 & 100 & 48 & 1.835 \\
400 & 200 & 79 & 1.835 & 400 & 300 & 80 & 1.835 \\
400 & 380 & 80 & 1.835 & 400 & 395 & 80 & 1.835 \\
450 & 300 & 38 & 0.948 & 450 & 350 & 39 & 0.948 \\
450 & 400 & 39 & 0.948 & 450 & 430 & 39 & 0.948 \\
450 & 445 & 39 & 0.948 & 500 & 1 & 25 & 0.518 \\
500 & 100 & 25 & 0.518 & 500 & 200 & 24 & 0.518 \\
500 & 300 & 25 & 0.518 & 500 & 350 & 25 & 0.518 \\
500 & 400 & 23 & 0.518 & 500 & 450 & 25 & 0.518 \\
500 & 480 & 25 & 0.518 & 500 & 495 & 25 & 0.518 \\
550 & 1 & 20 & 0.296 & 550 & 100 & 20 & 0.296 \\
550 & 200 & 20 & 0.296 & 550 & 300 & 20 & 0.296 \\
550 & 350 & 15 & 0.296 & 550 & 400 & 20 & 0.296 \\
550 & 450 & 15 & 0.296 & 550 & 500 & 20 & 0.296 \\
550 & 530 & 20 & 0.296 & 550 & 545 & 20 & 0.296 \\
600 & 1 & 14 & 0.175 & 600 & 100 & 15 & 0.175 \\
600 & 200 & 15 & 0.175 & 600 & 300 & 15 & 0.175 \\
600 & 350 & 14 & 0.174 & 600 & 400 & 15 & 0.175 \\
600 & 450 & 15 & 0.174 & 600 & 500 & 15 & 0.175 \\
600 & 580 & 15 & 0.175 & 600 & 595 & 15 & 0.175 \\
650 & 1 & 15 & 0.107 & 650 & 100 & 15 & 0.107 \\
650 & 200 & 15 & 0.107 & 650 & 300 & 15 & 0.107 \\
650 & 350 & 15 & 0.107 & 650 & 400 & 15 & 0.107 \\
650 & 450 & 15 & 0.107 & 650 & 500 & 15 & 0.107 \\
650 & 600 & 15 & 0.107 & 700 & 1 & 10 & 0.067 \\
700 & 100 & 10 & 0.067 & 700 & 200 & 8 & 0.067 \\
700 & 300 & 10 & 0.067 & 700 & 350 & 10 & 0.067 \\
700 & 400 & 10 & 0.067 & 700 & 450 & 10 & 0.067 \\
700 & 500 & 10 & 0.067 & 700 & 600 & 10 & 0.067 \\
750 & 1 & 10 & 0.043 & 750 & 100 & 10 & 0.043 \\
750 & 200 & 10 & 0.043 & 750 & 300 & 10 & 0.043 \\
750 & 350 & 8 & 0.043 & 750 & 400 & 10 & 0.043 \\
750 & 450 & 10 & 0.043 & 750 & 500 & 10 & 0.043 \\
750 & 600 & 10 & 0.043 & 800 & 1 & 25 & 0.028 \\
800 & 50 & 5 & 0.028 & 800 & 100 & 5 & 0.028 \\
800 & 150 & 5 & 0.028 & 800 & 200 & 5 & 0.028 \\
800 & 250 & 5 & 0.028 & 800 & 300 & 5 & 0.028 \\
800 & 350 & 5 & 0.028 & 800 & 400 & 5 & 0.028 \\
800 & 450 & 5 & 0.028 & 800 & 500 & 5 & 0.028 \\
800 & 550 & 5 & 0.028 & 800 & 600 & 5 & 0.028 \\
850 & 1 & 5 & 0.019 & 850 & 50 & 5 & 0.019 \\
850 & 100 & 5 & 0.019 & 850 & 150 & 5 & 0.019 \\
850 & 200 & 5 & 0.019 & 850 & 250 & 5 & 0.019 \\
850 & 300 & 5 & 0.019 & 850 & 350 & 5 & 0.019 \\
850 & 400 & 5 & 0.019 & 850 & 450 & 5 & 0.019 \\
850 & 500 & 5 & 0.019 & 850 & 550 & 5 & 0.019 \\
850 & 600 & 5 & 0.019 & 900 & 1 & 5 & 0.013 \\
900 & 50 & 5 & 0.013 & 900 & 100 & 5 & 0.013 \\
900 & 150 & 5 & 0.013 & 900 & 200 & 5 & 0.013 \\
900 & 250 & 5 & 0.013 & 900 & 300 & 5 & 0.013 \\
900 & 350 & 5 & 0.013 & 900 & 400 & 5 & 0.013 \\
900 & 450 & 5 & 0.013 & 900 & 500 & 4 & 0.013 \\
900 & 550 & 5 & 0.013 & 900 & 600 & 5 & 0.013 \\
950 & 1 & 5 & 0.009 & 950 & 50 & 5 & 0.009 \\
950 & 100 & 5 & 0.009 & 950 & 150 & 5 & 0.009 \\
950 & 200 & 5 & 0.009 & 950 & 250 & 5 & 0.009 \\
950 & 300 & 5 & 0.009 & 950 & 350 & 5 & 0.009 \\
950 & 400 & 5 & 0.009 & 950 & 450 & 5 & 0.009 \\
950 & 500 & 5 & 0.009 & 950 & 550 & 5 & 0.009 \\
950 & 600 & 5 & 0.009 & 1000 & 1 & 5 & 0.006 \\
1000 & 50 & 5 & 0.006 & 1000 & 100 & 5 & 0.006 \\
1000 & 150 & 5 & 0.006 & 1000 & 200 & 5 & 0.006 \\
1000 & 250 & 5 & 0.006 & 1000 & 300 & 5 & 0.006 \\
1000 & 350 & 5 & 0.006 & 1000 & 400 & 5 & 0.006 \\
1000 & 450 & 5 & 0.006 & 1000 & 500 & 5 & 0.006 \\
1000 & 550 & 5 & 0.006 & 1000 & 600 & 5 & 0.006 \\
\bottomrule
\end{tabular}
\end{tiny}
\end{center}
\end{table}

